Robust Stochastically-Descending Unrolled Networks

Deep unrolling, or unfolding, is an emerging learning-to-optimize method that unrolls a truncated iterative algorithm in the layers of a trainable neural network. However, the convergence guarantees and generalizability of the unrolled networks are still open theoretical problems. To tackle these problems, we provide deep unrolled architectures with a stochastic descent nature by imposing descending constraints during training. The descending constraints are forced layer by layer to ensure that each unrolled layer takes, on average, a descent step toward the optimum during training. We theoretically prove that the sequence constructed by the outputs of the unrolled layers is then guaranteed to converge for unseen problems, assuming no distribution shift between training and test problems. We also show that standard unrolling is brittle to perturbations, and our imposed constraints provide the unrolled networks with robustness to additive noise and perturbations. We numerically assess unrolled architectures trained under the proposed constraints in two different applications, including the sparse coding using learnable iterative shrinkage and thresholding algorithm (LISTA) and image inpainting using proximal generative flow (GLOW-Prox), and demonstrate the performance and robustness benefits of the proposed method.

==> sections/Notation.tex <==
\newpage
\section{Summary of Notations and Symbols}
In this section, we summarize all notations, mentioned in the text and appendices.
\begin{table}[h]
\centering
    \begin{tabular}{c l  c l  c l}
        $f_{\vartheta}(.)$ & global objective function  & $\cal D$  & data distribution  & $\boldsymbol{\Theta}$ & compact set \\
        $f_i(.)$ & local objective function & $\cal E$ & set of edges in $\cal G$ & $\boldsymbol{\Phi}(.)$ & learnable optimizer \\
        ${\bf h}_{l}$ & graph filter coefficients & $\cal F$  & sigma algebra  & $\boldsymbol{\Phi}_{\bf w}(.)$ & optimizer with \\
        $i, j$ & agent IDs & $\cal G$  & a graph &  & parameterization $\bf W$ \\
        $l$ & layer & $\cal H$  & hypothesis space & $\Omega$  & sample space  \\
        $t$ & discrete time variable & $\cal L$  & Lagrangian function & $\alpha$ & DGD step size \\
       ${\bf y}_i$ & local variable at $i$ & $\widehat{\cal L}$  & empirical Lagrangian  & $\alpha_k$ & stochastic process\\
       ${\bf y}_{l,i}$ & $l$-th layer's output at $i$ & $\cal N$ & Gaussian distribution & $\beta_k$ & stochastic process \\
       $B$ & constant & ${\cal N}_i$  & local neighborhood of $i$ & $\gamma$ & constant \\
       $C$ & Lipschitz constant & $\cal P$ & task distribution & $\delta $ & constant in $[0, 1)$\\
       $\widehat{D}$ & empirical dual value & $\cal T$ & task & $\epsilon$ & constant in $(0, 1)$ \\
       $K$ & no. of filter taps & $\cal V$  & set of nodes in $\cal G$ & $\zeta(.)$ & sample complexity  \\
        $L$ & no. of unrolled layers & ${\cal W}_l$  & Gaussian distributions & $\eta$ & constant \\
        $M$ & Lipschitz constant & ${\mathfrak{F}}$  & a function class & $\boldsymbol{\theta}$ & parameterization of $\mathfrak{F}$ \\
        ${\bf M}_l$ & MLP weights of $l$-th layer & $\widehat{\mathbb{E}}[.]$  & sample average &  $\boldsymbol{\vartheta}$ & input data \\
        $N$ & no. of agents & $\mathbb{R}$  & real numbers & $\boldsymbol{\lambda}$ & dual variable \\
        ${\bf N}_l$ & noise added to ${\bf Y}_{l-1}$ & $\times$  & cartesian product  & $\mu_u, \mu_\lambda$ & priaml-dual step sizes \\
        $P$ & probability measure & $\|.\|$  & $\ell_2$/Frobenius norm &  $\mu_0$ & mean of ${\bf Y}_0$ \\
        $Q$ & sample size & $(.)^*$ & optimal value  &  $\nu$ & constant \\
        ${\bf S}$ & graph shift operator  & $\nabla$ & gradient & $\rho$ & constant  \\
        $X$ & random variable  & $\mathbf{1}\{.\}$ & indicator function  & $\sigma$ & nonlinear activation  \\
        ${\bf Y}_l$ & output at unrolled layer $l$  & $\ell(.)$ & loss function & $\sigma_l$ & noise variance \\
        ${Z}_l$ & average gradient norm &  &  & $\omega$ & element in $\Omega$ \\
        ${Z}_l^\text{best}$ & lowest value of $Z_l$  &  &  & $\omega_{ij}$ & graph weight  \\
        
       
    \end{tabular}
\end{table}
